Fast Light-Weight Near-Field Photometric Stereo

We introduce the first end-to-end learning-based solution to near-field Photometric Stereo (PS), where the light sources are close to the object of interest. This setup is especially useful for reconstructing large immobile objects. Our method is fast, producing a mesh from 52 512$\times$384 resolution images in about 1 second on a commodity GPU, thus potentially unlocking several AR/VR applications. Existing approaches rely on optimization coupled with a far-field PS network operating on pixels or small patches. Using optimization makes these approaches slow and memory intensive (requiring 17GB GPU and 27GB of CPU memory) while using only pixels or patches makes them highly susceptible to noise and calibration errors. To address these issues, we develop a recursive multi-resolution scheme to estimate surface normal and depth maps of the whole image at each step. The predicted depth map at each scale is then used to estimate `per-pixel lighting' for the next scale. This design makes our approach almost 45$\times$ faster and 2$^{\circ}$ more accurate (11.3$^{\circ}$ vs. 13.3$^{\circ}$ Mean Angular Error) than the state-of-the-art near-field PS reconstruction technique, which uses iterative optimization.

==> latex/content/Ablation.tex <==
\vspace{-2em}
\section{Ablation}
\label{sec:ablation}
We analyze the importance of per-pixel lighting estimation as input to the normal prediction network with an ablation study. 

\textbf{Importance of Per-Pixel Lighting} We train a variant of our network that does not require per-pixel lighting estimation as input to the normal estimation network. Concretely, rather than using the per-pixel lighting $A^j_i$ and $L^j_i$ as input to the network $G_{IN}$ and $G_{RN}$ we only input the lights' parameters $p^j,d^j,\mu^j$ at each pixel. Note that, these light parameters are associated with global lighting conditions and do not reflect per-pixel lighting effects unlike $A^j_i$ and $L^j_i$. We observe that explicitly estimating and using per-pixel lighting as input improves the performance from X to Y. This also shows that a more direct adoption of the recursion idea presented by Lichy \textit{et al.} in \cite{Lichy_2021_CVPR} from far-field to near-field PS, if less effective without using per-pixel lighting estimation.


\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
       & MAE & MZE \\ \hline
     with per-pixel lighting estimation & \textbf{11.32} & \textbf{4.43} \\
     w/o per-pixel lighting estimation & 14.88 & 4.89 \\
     \hline
    \end{tabular}
    \vspace{-1em}
    \caption{We show that using per-pixel lighting as input to the recursive normal prediction network improves prediction accuracy.}
    \label{tab:ablation}
    \vspace{-1em}
\end{table}


\textbf{Recursive Inference vs Bilinear Upsampling.} Our model gives an estimate of normals and depth at all resolutions, starting from 64, 128 to the input resolutions. In Table \ref{tab:ang_err_upsampling} we take the predictions of our network at a certain resolution (64, 128, 256, 512, and 1024) and then bilinearly upsample them to 2048 resolution. This demonstrates that applying our network recursively is doing more than simply bilinearly upsampling the predicted normal and depth map from low to high resolution.


\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
     \hline
        Resolution &  64 & 128 & 256 & 512 & 1024 & 2048 \\ \hline 
        MAE & 16.8 & 14.0 & 12.4 & 11.6 & 11.32 & 11.32 \\
       MZE & 15.2 & 8.2 & 5.7 & 4.8 & 4.5 & 4.4
        \\ \hline
    \end{tabular}
    \vspace{-0.5em}
    \caption{ We bilinearly upsample the predictions of our network at each resolution (presented in the columns) to 2048 and evaluate the MAE and MZE metrices to demonstrate that the recursive predictions are doing much more than naive bilinear upsampling.}
    

    \label{tab:ang_err_upsampling}
    \vspace{-0.5em}
\end{table}

==> latex/content/teaser.tex <==
% teaser.tex is referenced in cvpr.cls
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\includegraphics[width=.95\textwidth]{latex/content/figures/teaser_v3.png}
\vspace{-1em}
%
\captionof{figure}{We present a fast light-weight approach for solving near-field Photometric Stereo (PS), which is particularly useful for capturing large objects, e.g. a sofa, in a small confined space. We capture an object with an iPhone camera and a handheld flashlight. Our method is significantly faster during inference and produces more accurate reconstructions than existing methods S20~\cite{santo2020deep} and L20~\cite{Logothetis2020ACB}.}
\label{fig:teaser}

